Improved Approximations for Stationary Bipartite Matching: Beyond Probabilistic Independence

We study stationary online bipartite matching, where both types of nodes--offline and online--arrive according to Poisson processes. Offline nodes wait to be matched for some random time, determined by an exponential distribution, while online nodes need to be matched immediately. This model captures scenarios such as deceased organ donation and time-sensitive task assignments, where there is an inflow of patients and workers (offline nodes) with limited patience, while organs and tasks (online nodes) must be assigned upon arrival. We present an efficient online algorithm that achieves a $(1-1/e+\delta)$-approximation to the optimal online policy's reward for a constant $\delta > 0$, simplifying and improving previous work by Aouad and Sarita\c{c} (2022). Our solution combines recent online matching techniques, particularly pivotal sampling, which enables correlated rounding of tighter linear programming approximations, and a greedy-like algorithm. A key technical component is the analysis of a stochastic process that exploits subtle correlations between offline nodes, using renewal theory. A byproduct of our result is an improvement to the best-known competitive ratio--that compares an algorithm's performance to the optimal offline policy--via a $(1-1/\sqrt{e} + \eta)$-competitive algorithm for a universal constant $\eta > 0$, advancing the results of Patel and Wajc (2024).

==> analysis_old.tex <==


\section{Improved Approximation Ratio Analysis}\label{sec:approximation}



For some impatient types the above analysis may already be loose; we concretely identify such cases below in what we refer to as the ``case disjunction." These bounds are also useful for analyzing the \emph{competitive ratio} against the optimum offline benchmark, as we show in \Cref{sec:competitiveRatio}. We first fix some notation used in the remainder of this section. 

\paragraph{Notation.} In the below discussion let $\textsf{ALG}_j$  denote the expected stationary reward of \Cref{alg:corrprop} from matches to $j \in J$. For any $S \subseteq J$ we let $\textsf{Gain}_S := \sum_{j \in S} \sum_{i \in V} r_{i,j} x_{i,j}$ denote the total gain from matching to online types in $S$ in the optimal LP solution. For convenience of notation, we will let $\textsf{Gain}_j := \textsf{Gain}_{\{j\}}$. For any offline type $i$, we let $N_i := \{ j : x_{i,j} > 0 \}$ denote the neighborhood of $i$ (and define $N_j$ analogously). 

\subsection{The Case Disjunction}

In the following, let $\epsilon > 0$. For ease of exposition we also will not concern ourselves with optimizing the constant resulting in the analysis. Below we fix some impatient type $j \in J$ and identify two cases where \Cref{alg:corrprop} achieves a better-than-$(1-1/e)$ approximation on $j$. 


\paragraph{Case 1: \eqref{TLPon} does not fill $j$ at its arrival rate.} 
\begin{obs} \label{obscase1}
If $\sum_{i} x_{i,j}/\gamma_i \le 1-\epsilon $, then $\textup{\textsf{ALG}}_j \ge (1 - 1/e + c(\epsilon)) \cdot \textsf{\textup{Gain}}_j$ for some $c(\epsilon) > 0$. 
\end{obs}
\begin{proof} Recall from \eqref{eqn:1minusexpbound} our lower bound
    \begin{align*}
        \textsf{ALG}_j &\ge \gamma_j \cdot \int_0^{\infty} \E [ \min(1, R_j(w )] \, dw 
        \ge \gamma_j \cdot \int_0^{\infty} \left( 1 - \exp \left(-\sum_{i : r_{i,j} \ge w} x_{i,j}/\gamma_j \right) \right) \, dw.
    \end{align*}
    For convenience we define the function $g(\cdot)$ such that $1 - \exp(-z) = (1 - 1/e + g(z)) \cdot z$ and note that $g(\cdot)$ is positive and decreasing for $z \in (0,1)$. We then can bound 
 \begin{align*}
        \textsf{ALG}_j \ge \gamma_j \cdot \int_0^{\infty} \left( 1 - 1/e + g(1 - \epsilon ) \right) \cdot \left( \sum_{i : r_{i,j} \ge w}  x_{i,j} / \gamma_j \right)  \, dw = (1 - 1/e + g(1 - \epsilon )) \cdot \textsf{Gain}_j
    \end{align*} as claimed.
\end{proof}

\paragraph{Case 2: \eqref{TLPon} does not fill $j$ at a single reward weight.} 
\begin{obs}\label{lem:bounded_match_rate}
    Let $\textup{\textsf{Gain}}_j := \sum_i x_{i,j} \cdot r_{i,j}$ and for real numbers $a \le b$ define $\textup{\textsf{Gain}}_j^{[a,b]} := \sum_{i : r_{i,j} \in [a,b]} x_{i,j} \cdot r_{i,j}$. Suppose that for every $w \in \mathbb{R}$ we have $\textup{\textsf{Gain}}_j^{[w, w(1+\epsilon)]} < (1-\epsilon) \cdot \textup{\textsf{Gain}}_j$. Then, we have $\textup{\textsf{ALG}}_j \geq (1-1/e+c(\epsilon)) \cdot \textup{\textsf{Gain}}_j$, for $c(\epsilon ) > 0$. 
\end{obs} 
\begin{proof}

    
    Let $w^*$ be the weight such that $j$ has a $\epsilon / 2$ fraction of its LP-weighted gain sent to rewards in $[0, w^*]$; formally, define $$w^* := \inf \left\{ w \ge 0:  \frac{\textsf{Gain}_j^{[0, w]}}{\textsf{Gain}_j} \ge \epsilon / 2 \right\}.$$ By assumption we know that $j$ sends at most a $1-\epsilon$ fraction of its LP-weighted gain mass in the interval $[w*, (1+\epsilon) w^*].$ Thus the fraction of LP-weighted gain $j$ has from rewards in the interval $((1+\epsilon) w^*, \infty)$ is lower bounded by $\epsilon/2.$ Also, because $\textsf{LP}_j^{[0,w^*]} \ge \epsilon/2 \cdot \textsf{LP}_j$, we can observe that $$\sum_{i : r_{i,j} \in [0, w^*]} x_{i,j}   \ge \epsilon/2 \cdot \sum_{i} x_{i,j}.$$ If $\sum_{i} x_{i,j} / \gamma_j \le 1 - \epsilon $ we are already done by Case 1; so we assume $\sum_{i} x_{i,j} / \gamma_j > 1 - \epsilon$ which implies that for any $w > w^*$, we have $$\sum_{i : r_{i,j} \ge w} x_{i,j} / \gamma_j \le 1 - \epsilon (1-\epsilon) /2.  $$
    Now, we bound
    \begin{align*}
        \textsf{ALG}_j 
        &\ge \gamma_j \cdot \int_0^{\infty} \left( 1 - 1/e + g \left( \sum_{i: r_{i,j} \ge w} x_{i,j} / \gamma_j \right) \right) \cdot \left( \sum_{i : r_{i,j} \ge w}  x_{i,j} / \gamma_j \right)  \, dw \\
        &\ge \gamma_j \cdot \int_0^{\infty} \sum_i (1 - 1/e + g(1 - \epsilon (1-\epsilon) /2) \cdot \mathbbm{1}[w > w^*]) \cdot x_{i,j}/\gamma_j \cdot \mathbbm{1}[w \le r_{i,j}] \, dw \\
        &= (1-1/e) \cdot \textsf{LP}_j +  g(1 - \epsilon (1-\epsilon) /2) \cdot \sum_i x_{i,j} \cdot  \max(0, r_{i,j} - w^*) \, dw \\
        &\ge (1-1/e) \cdot \textsf{LP}_j +  g(1 - \epsilon (1-\epsilon) /2) \cdot \sum_{i : r_{i,j} \ge (1+\epsilon)w^*} x_{i,j} \cdot r_{i,j} \cdot \epsilon/2   && (\epsilon \le 1) \\
        &= (1-1/e) \cdot \textsf{LP}_j +  g(1 - \epsilon (1-\epsilon) /2) \cdot \textsf{LP}_j^{[(1+\epsilon)w^*,\infty)} \cdot \epsilon/2  .
    \end{align*}
    Recalling that $\textsf{LP}_j^{[(1+\epsilon)w^*,\infty)} > \epsilon / 2 \cdot \textsf{LP}_j$ concludes the argument. 
\end{proof}

\paragraph{Case 3: Some of $j$'s proposal probabilities $\{P_{i,j}\}$ are bounded away from 1.}


\begin{obs}\label{lem:bounded_proposal}
    Suppose there exists $S \subseteq I$ such that $\sum_{i \in S} \frac{x_{i,j}}{\gamma_j} \ge \epsilon$ and $\max_{i \in S} P_{i,j} \leq 1-\epsilon$. Then, we have $\textup{\textsf{ALG}}_j \geq (1-1/e+c(\epsilon)) \cdot \textup{\textsf{Gain}}_{j}$ for some $c(\epsilon) > 0$.
\end{obs} 
\begin{proof}

We recall the bound \begin{align*}
 \textsf{ALG}_j &\ge \gamma_j \cdot \int_0^{\infty} \E [ \min(1, R_j(w)] \, dw.
 \end{align*} For any $w > 0$, let $I_w$ denote the set of $i \in I$ with reward $r_{i,j} \ge w$. Let $\mu_w := \sum_{i \in I_w} x_{i,j} / \gamma_j$ and let $\mu_{w, S} := \sum_{i \in I_w \cap S} x_{i,j} / \gamma_j$. In the convex order, we have by \Cref{lem:weightedPoisCvx} that \begin{align*}
       R_{j}(w) = \sum_{i \in I_w} P_{i,j} \cdot \textup{Pois}(x_{i,a} / \mu_i ) & \cvxle  \sum_{i \in I_w \cap S} (1-\epsilon) \cdot \textup{Pois}\left(\frac{x_{i,a} \cdot P_{i,j}}{1-\epsilon}\right) +  \sum_{i \in I_w \setminus S} 1 \cdot \textup{Pois}\left(x_{i,a} \cdot P_{i,j} \right).
    \end{align*}
As $P_{i,j} := \frac{x_{i,j} / \gamma_j}{x_{i,a} / \mu_i}$ the RHS is distributed exactly as $(1-\epsilon) \cdot \text{Pois} \left( \frac{\mu_{w,S}}{1-\epsilon} \right) + \text{Pois} \left( \mu_w - \mu_{w,S} \right).$ For convenience denote this distribution by $D$; we then have the stationary probability $j$ is matched is 
\begin{align*}
\mathbb{E}[\min(1, R_j(w))] 
    &\ge \mathbb{E}[\min(1, D)] \\
    % &= (1 - \exp(-\mu_w + \mu_{w,S})) \cdot 1 + \exp(-\mu_w + \mu_{w,S}) \cdot \mathbb{E} \left[  \min \left( 1, (1-\epsilon) \cdot \text{Pois} \left( \frac{\mu_{w,S}}{1-\epsilon} \right)  \right) \right] \\
    &= 1 - \exp(-\mu_w + \mu_{w,S}) \cdot \mathbb{E} \left[ \max \left(0, 1 - (1-\epsilon) \cdot \text{Pois} \left( \frac{\mu_{w,S}}{1-\epsilon} \right)  \right) 
    \right]  
\end{align*}

Note that when $\mu_w = 1$ and $\mu_{w,S} = 0$, the RHS is precisely when $1-1/e$; when either $\mu_w < 1$ or $\mu_{w,S} > 0$ this is loose. By the assumption of this case, we know $\mu_w - \mu_{w,S} \le 1 - \epsilon$; from this it is straightforward to see $ \mathbb{E}[\min(1,R_j(w))] \ge (1-1/e + c(\epsilon)) \cdot \mu_w$ (for a full proof, refer to \Cref{app:expectationbounding}). The claim then follows from direct computation:
\begin{align*}
    \textsf{ALG}_j &\ge \gamma_j \cdot \int_0^{\infty} \E [ \min(1, R_j(w)] \, dw \\
    &\ge \gamma_j \cdot (1 - 1/e + c(\epsilon)) \cdot \int_0^{\infty} \mu_w \, dw =  (1 - 1/e + c(\epsilon)) \cdot \textsf{Gain}_j. \qedhere
\end{align*}


\end{proof}

In summary, the three cases above identify scenarios where \Cref{alg:corrprop} beats the $1-1/e$ bound on a fixed online type $j$. If a constant fraction of the LP reward is supported on online types $j$ falling into one of these cases, then \Cref{alg:corrprop} beats $1-1/e$, as formalized in the following observation. We treat $\eps,\delta>0$ as fixed constants, chosen sufficiently small relative to the constant factor gain in the approximation ratio that we establish below.
\begin{obs} \label{obs:casesBeat1-1/e}

    Let $A$ denote the set of all online types $j$ such that at least one of Case 1, 2, or 3 hold. If $\textup{\textsf{Gain}}_A \geq \epsilon \cdot \textup{\textsf{Gain}}_J$, then \Cref{alg:corrprop} achieves staionary reward at least $(1 - 1/e + c(\epsilon)) \cdot \textup{\textsf{Gain}}_J$ for some constant $c(\epsilon) > 0$. 
\end{obs}

%Hence  we focus on $B := J \setminus A$ with the assumption 
%\begin{align}\label{asmp:set_b_bound}
%    \textsf{LP}_B \geq (1-\epsilon) \cdot \textsf{LP}_J \ .
%\end{align}
%For each $j \in B$, we have that $\sum_i \frac{x_{i,j}}{\gamma_j} \ge 1 - \epsilon$, and that there exists some $S_j \subseteq I$ such that  $\sum_{i \in S_j} \frac{x_{i,j}}{\gamma_j} \ge 1 - \epsilon$ and $P_{i,j} \ge 1-\epsilon$ for every $i \in S_j$. \Alicomment{So $x_{i,j}>0$ for all $i\in S_j$}

\subsection{Large-Degree Case: Beyond Independent Queues}
A key limitation of our analysis is using the virtual Markov chain `vMc' to lower bound the availability of offline vertices. \todo{Link to appendix with example where vMc is stuck at $1-1/e$.} In vMc, the queue lengths are mutually independent across offline nodes. Here, we seek to develop a refined lower bound, which yields an improved approximation ratio in the hard case. As before, in this subsection we treat $\eps >0$ as fixed constants, chosen sufficiently small relative to the constant factor gain in the approximation ratio that we establish below.

For many inputs, the case disjunction shows that \Cref{alg:corrprop} achieves a better than $(1-1/e)$-approximation to optimum online; we assume for the remainder of this subsection that we are not in such a scenario, as formalized in \Cref{obs:casesBeat1-1/e}. In particular, this means that if $B$ denotes the set of all online types such that none of Case 1, 2, or 3 hold, we have $\textsf{Gain}_{B} \ge (1 - \epsilon) \cdot \textsf{Gain}_J$. Note that for every $j \in B$, we have  
$$ \text{(i)  there exists } S_j \subseteq I \text{  with } \sum_{i \in S_j} x_{i,j} / \gamma_j \ge 1 - 2 \epsilon \text{ and } \min_{i \in S_j} P_{i,j} \ge 1 - \epsilon \text{ (via Case 1 and 3)} $$ and 
$$\text{(ii) there exists some }r_j \text{ such that } \textsf{Gain}_j^{[r_j, r_j( 1 + \epsilon ) ]} \ge (1 - \epsilon ) \cdot \textsf{Gain}_j \text{ (via Case 2)}.$$

This lets us ``clean'' our LP solution before moving to the meat of our analysis. We first remove all online types not in $B$. For every $j \in B$, we will then remove any edge to some $i$ with $r_{i,j} \notin [r_j, r_j ( 1 + \epsilon )]$. For ease of analysis, for any remaining edge $i \sim j$ we will lower the reward $r_{i,j}$ to $w_j$. Finally, we will remove any edge $i \sim j$ if $i \notin S_j$. It is easy to see that these four changes in total lead to LP solution with objective value at least $(1-4 \epsilon) \cdot \textsf{Gain}_J$. This is summarized as our first ``parameter assumption" below.

\begin{enumerate}[label=(PA-\arabic*)]%uses package enumitem
    \item The rewards are online vertex-weighted with $r_{i,j}=r_j$. For every $i \in N_j$, we have $P_{i,j} := \frac{x_{i,j} / \gamma_j}{x_{i,a} / \mu_i } \ge 1 - \epsilon$, and $\sum_{i \in N_j} x_{i,j} / \gamma_j \ge 1 - \epsilon$. \label{structuralassumption}
 \end{enumerate}

 Before moving on to the next parameter assumptions, we briefly establish a few consequences the constraints of \eqref{TLPon} imply in this regime. Firstly, observe that because $P_{i,j} \le 1$ (Constraint \eqref{eqn:tightOnlineConstraint}) we have
 \begin{align}
     \sum_{i \in N_j} \frac{x_{i,a}}{\mu_i} &\ge \sum_{i \in N_j} \frac{x_{i,j}}{\gamma_j} \ge 1 - \epsilon .
 \end{align}
Additionally, by Constraint~\eqref{eqn:tightOnlineFlow} of \eqref{TLPon} we have
\begin{align}
 \sum_{i \in N_j} \frac{\lambda_i}{\mu_i } &\ge \log \left( \frac{1}{\epsilon} \right).
\end{align}

Finally, Constraint~\ref{eqn:tightOfflineFlow} along with $P_{i,j} \in [1-\epsilon, 1]$ for $j \in N_i$ imply 
\begin{align}
(1-\eps) \cdot \frac{\gamma_j \lambda_i}{\mu_i + \sum_{k \in N_i} \gamma_k} \leq x_{i,j} \leq \frac{1}{1-\eps} \cdot \frac{\gamma_j \lambda_i}{\mu_i + \sum_{k \in N_i} \gamma_k} \quad \text{ for } i \in I, j \in N_i \label{ineq:match_bound}
\end{align}
and \begin{align}
    \frac{\mu_i\lambda_i}{\mu_i + \sum_{k \in N_i} \gamma_k} \leq x_{i,a} \leq \frac{1}{1-\eps} \cdot \frac{\mu_i\lambda_i}{\mu_i + \sum_{k \in N_i} \gamma_k} \quad \text{for } i \in I. \label{ineq:abandonment_bound}
\end{align}

Refer to \Cref{xijxiabounds} for a proof. 

 The remaining parameter assumptions depend on the following definition, where we split the offline types into two halves called ``top'' and ``bottom.''

 \paragraph{Top and Bottom Types.} Fix $j\in [m]$.  We refer to $i\in [1, \lceil \frac{n}{2} \rceil -1] = \topp$ as the top types and $i\in [\lceil \frac{n}{2} \rceil, n]=\bott$ as the bottom types. For every $i\in [n]$ and $j\in [m]$, we use $N_i := \{j\in [m]: x_{i,j}>0\}$ for each $i\in [n]$ and similarly $N_j := \{i \in [n]: x_{i,j} > 0\}$. For convenience, we let $N_j^{\uparrow} := N_j \cap \topp$ and $N_j^{\downarrow} := N_j \cap \bott$. \\


With this definition in place, we are ready to state our two remaining parameter assumptions. 

\begin{enumerate}[label=(PA-\arabic*)]%uses package enumitem
\setcounter{enumi}{1}


\item The instance is  processed such that $\max_{i\in [n]} \lambda_i/\mu_i \leq \eps^2$. Specifically, via the superposition property of Poisson processes, we can dilute type $i$ (with arrival rate $\lambda_i$) into $\lceil \frac{\lambda_i}{\epsilon^2 \mu_i} \rceil$ copies, each with arrival rate at most $\epsilon^2 / \mu_i$. 

\item For every $j\in B$, the instance is {\em $j$-balanced}, meaning that $ \sum_{i\in N_j^\uparrow} \lambda_i = \frac{1}{2} \cdot \sum_{i\in N_j} \lambda_i$. Again, this is easy to enforce via splitting: for any patient type $i$, we can split it into two arrival processes each with rate $\lambda_i/2$, one in TOP and one in BOT. 

\end{enumerate}

\paragraph{Greedy Algorithm.} As every proposal probability is at least $1-\epsilon$, for convenience of the analysis we will analyze the greedy algorithm, which matches an arriving $j$ to a present offline type of minimum index. equivalent to \Cref{alg:corrprop} with every reward equal to 1. \todo{Easy to see this is equivalent to corr prop (?)}







% \item Queues are truncated to be binary, i.e., $\prpar{\tilde{Q}^\pi_i \leq 1} = 1$ for every policy $\pi$, which comes with a small loss in the approximation ratio. In what follows, we overload our original notation and still use $Q^\pi$ to denote the truncated process.
% Note that for a tie-breaking proposal-based algorithm, this amounts to deleting matches of type-$i$ offline nodes at rate $\eps^2 \lambda_i$ (since $\prpar{Q^\pi_i \geq 1} = \eps^2$ in the real process) uniformly over all $j$-s.


 
\begin{comment}

\paragraph{The algorithmic reduction to balancedness.} Property 3 is new and we now provide an algorithm to achieve it. Suppose we rearrange the offline node indices by drawing a permutation $\sigma$ uniformly at random. By Theorem 3.1 in~\cite{adamczak2016circular}, there exists a universal constant $c>0$, such that for all $j \in B$, we have
\begin{eqnarray*}
\prtwo{\sigma}{\left|\sum_{i\in S_j^\uparrow} \lambda_i - \frac{1}{2} \sum_{i\in S_j}\lambda_i \right| \Alirezaedit{\geq} \eps \sum_{i\in S_j}\lambda_i} \leq 2^{-c \frac{1}{\eps2}  (\sum_{i\in S_j}\lambda_i)} \leq \eps^2 \ ,
\end{eqnarray*}
where we choose $\eps$ sufficiently small relative to the constant $c$. Similarly, we have 
\begin{eqnarray*}
\prtwo{\sigma}{\left|\sum_{i\in S_j^\uparrow} x_{i,a} - \frac{1}{2} \sum_{i\in S_j}x_{i,a} \right| \Alirezaedit{\geq} \eps } \leq 2^{-c \frac{1}{\eps^2}  } \leq \eps^2 \ .
\end{eqnarray*}
After drawing $\sigma$, our algorithm discards each $j\in B$ if they violate Property 4. By the union bound, this occurs with probability at most $2\eps^2$. Therefore, in expectation, the discarding operation reduces the approximation ratio by a small factor $O(\eps^2)$. Our algorithm then uses the ordered tie breaking with respect to $\sigma$ as in Property 5. In the sequel, we overload notation and use $B$ to denote all online types that survive the discarding operation. 

\Alirezacomment{couldn't we just split every offline node into two new nodes and form the two groups? No need for the random permutation and we would just use an arbitrary ranking s.t. group preservation} \Alicomment{Yes! I completely missed this. The use of random permutation concentration is an overkill, sorry. But it's a cool tool. Please edit the above part}
\end{comment}
Now, our goal is to develop a tighter analysis of the expected average match rate for each offline type $j\in B$.


\paragraph{The semi-virtual Markov chain.} First, note that we can truncate the queues to be binary, i.e., $\prpar{\tilde{Q}^\pi_i \leq 1} = 1$ for our policy $\pi$, at the cost of a small loss $O(\eps^2)$ in the approximation ratio. To justify this, observe that the probability of empty queues under vMc is
\begin{eqnarray}
\prtwo{v}{\sum_{i\in S_j}\tilde{Q}^\pi=0} &=& \prod_{i\in S_j} \left(1-\frac{\lambda_i}{1+\lambda_i+\sum_{k\in N_i}\gamma_k} \right) \nonumber\\
& \leq & \exp\left(-\sum_{i\in S_j} \frac{\lambda_i}{1+\lambda_i+\sum_{k\in N_i}\gamma_k} + \frac{\eps^2}{2}\frac{\lambda_i}{1+\lambda_i+\sum_{k\in N_i}\gamma_k}\right)\nonumber\\
& =& \frac{1}{e}+O(\eps^2) \approx \frac{1}{e} \label{approx:trunc}\ ,
\end{eqnarray}
where the inequality follows from Property 1. This is an alternative calculation for~\eqref{eqn:expectedmin1Rjw}, with a small approximation from imposing binary queues.  In what follows, approximation errors  resulting from this assumption are assumed to be negligible, and thus, denoted by $\approx$.
% Since the imposition of binary queues is inconsequential for the analysis, 
% we use $\approx$ for the resulting approximations.
 We also overload our original notation and still use $Q^\pi$ to denote the truncated queueing process. 


To analyse the expected average match rate for type $j$ online nodes, we introduce a new approximation.  Consider the Markov modulated process `sMc' (indexed by `s') specified as follows:
\begin{enumerate}
\item The marginal distribution $\prpartwo{s}{\{Q^s_i(t):i\in \topp\} \in \cdot} = \prpartwo{v}{\{Q^v_i(t):i\in \topp\} \in \cdot}$ follows the same distribution as the vMc. That is, the top offline vertices  have mutually independent queue lengths that evolve according to their respective birth-death process.

\item Let $\psi_j(t)\in \{0,1\}$ be the binary process for $\psi_j(t) = 1-{\bb I}[\sum_{i\in \topp \cap S_j} Q^s_i(t) > 0 ]$. When $\psi_j(t)=0$, a type $j$ arriving vertex is matched to a top offline vertex, and thus, it cannot be matched to a bottom offline vertex. To reflect this, let ${Q}^s_i(t)$ be the Markov modulated queueing process where (1) offline vertices of type $i$ arrive with rate $\lambda_i$ and abandon with rate $\mu_i=1$, and (2) the queue is depleted (when $Q^s_i(t) > 0$)  at rate $\sum_{j\in N_i} \psi_j(t) \gamma_j$.
\end{enumerate}

The steady-state queue lengths satisfy the following stochastic dominance relationships.

\begin{claim}
We have $Q\succeq_{st} Q^s \succeq_{st} Q^v$.
\end{claim}

While the analysis of vMc shows an upper bound $\prpartwo{v}{\sum_{i\in S_j}Q^v_i=0} \leq 1/e$, we prove that under sMc, there is a  strictly larger probability to match the arriving type $j$ vertex with an available offline vertex in $S_j$.
\begin{lemma} \label{lem:proof main}
Fix $j\in [m]$. There exists a constant $c>1$ such that $\prpartwo{s}{\sum_{i\in S_j}Q^s_i=0} \leq 1/(ce)$.
\end{lemma}
The remainder of this section tries to prove Lemma~\ref{lem:proof main}. Firstly, we note that 
\begin{eqnarray} \label{ineq:balanced}
 e^{-\frac{1}{2}-\eps} \leq \prtwo{s}{\sum_{i\in S_j^\uparrow}Q^s_i=0} = \exp\left(-\sum_{i\in S_j^+} x_{i,a}\right) \leq e^{-\frac{1}{2}+\eps} \ .
\end{eqnarray}
where the inequality follows from $j$-balancedness.

\paragraph{Bounds on the unmatched rate.} Consider an arbitrary time point $t^\infty$ in steady state and suppose that $\psi_j(t^\infty) = 1$. Think of $t^\infty$ as the time where an online vertex arrive of type $j$ arrives, and from the PASTA property, it sees the system in its average state. For each $i \in [n]$, indicate by $A_i(t)\in \{0,1\}$ whether an offline vertex of type $i$ has arrived and not reneged yet at time $t$, not accounting for previous matches, which implies $A_i(t) \geq Q_i(t)$. The arrivals and reneging departures of each  type $i\in \bott$ are independent of $\{Q_i^s: i\in \topp\}$ and the arrivals of online vertices.  Thus, we have $\prpar{A_i(t^\infty)=1| \psi_j(t^\infty) = 1} = \prpar{A_i(t^\infty)=1}= \frac{\lambda_i}{\mu_i+\lambda_i}$. In addition, let $t_i$ be the random time that has elapsed since the latest arrival. Since the process $\{A_i(t)\}_t$ is time-reversible (as a birth-death process), we can look at the process backward in time to obtain $t_i \sim Exp(\mu_i + \lambda_i)$.  \footnote{comment on $t^\infty$.}

Finally, for each $j\in [m]$, we introduce the random variable $\delta_{i,j} = \int_{t^\infty-t_i}^{t^\infty} \psi_j(t) dt$ that measures the total time $s$ elapsed in the interval $[t^\infty-t_i,t^\infty]$ during which $\sum_{i\in S_j^\uparrow}Q^s_i(s)=0$. This is the total time spent by the system of top queues in busy periods since the latest arrival of type $i$.

Lemma~\ref{lem:proof main} is proved if we manage to show that there exists a constant $c>1$ such that
\begin{eqnarray}
    && \ex{\left.\prod_{i\in S_j^\downarrow} \left(1- \frac{\lambda_i}{1+\lambda_i}\cdot \exp\left(-\sum_{k\in N_i} \gamma_k \delta_{i,k}\right)   \right)\right| \psi_j(t^\infty) = 1} \nonumber\\
    &&\quad \leq \frac{1}{c}\ex{\prod_{i\in  S_j^\downarrow} \left(\left. 1- \frac{\lambda_i}{1+\lambda_i}\cdot \exp\left(-\sum_{k\in N_i} \gamma_k t_i\right)\right)\right| \psi_j(t^\infty) = 1} \label{ineq:proba_hard} \\
    &&\quad \approx \frac{1}{ce} \exp\left(\sum_{i\in S_j^\uparrow} x_{i,a}\right) \ . \nonumber
\end{eqnarray}
% \Alirezacomment{If $N_i$-s overlap the LHS of (16) is not accurate? I think it is the worst-case so we're still fine?}\Alicomment{Good question! This is a subtle point in the construction of sMC. The LHS is exact even when $N_i$-s overlap because we assume that each $j$ has multiple copies in its busy periods (that's also a necessary simplification for the analysis). This is what I meant by the explanation below: ``Note that in busy periods, sMc still use online nodes' virtual copies to enforce the death rate.'' I should add a death rate of $\gamma_j$ for all $i$-s simultaneously (so the total rate is  $k\gamma_j$ where $k$ is the number of bottom $i$-s for which $j$ is in a busy period). This is also implied in (2) of the definition of sMc. Does it make sense?}

To unpack this expression, we note that the left-hand side calculates the probability that the arriving $j$ vertex cannot be matched with any bottom queue (in the modified instance) because the latest has either abandoned or been previously matched.\footnote{First, we draw $A_i(t^\infty)=0$ with probability $\frac{1}{1+\lambda_i}$, in which case $j$ cannot be matched with $i$. With the residual probability $\prpar{A_i(t^\infty)=1}=\frac{\lambda_i}{1+\lambda_i}$, we draw $t_i$-s and $\delta_{i,j}$-s and, conditional on their realizations, we calculate the probability that there has been no arrival in the set $N_i$ during the busy periods of each queue $i\in S^\downarrow_j$. Each queue has independent arrivals (virtual copies). } (Note that in busy periods, sMc still uses virtual copies of the online vertices to enforce the death rate of $\gamma_j$ for each $i$ in a busy period.) The right-hand side expression in~\eqref{ineq:proba_hard} corresponds to a similar probabilistic analysis for the vMc process. The conditioning on $\{\psi_j(t^\infty)=1\}$ does not alter that expression because $t_i$-s are independent of the system of top queues, and therefore, the last inequality follows from~\eqref{approx:trunc}.
% Simple algebra shows that this is an alternative calculation for~\eqref{eqn:expectedmin1Rjw}, with a smaller approximation from assuming that each queue contains at most one vertex. 
% In subsequent analysis, approximation errors resulting from this assumptions are assumed to be negligible.

We need to argue that $\delta_{i,k}$ is ``typically'' at least a constant-factor smaller than $t_i$. However, proving inequality~\eqref{ineq:proba_hard} is challenging because the random durations $\delta_{i,j}$ could be positively correlated, including with the event $\{\psi_j(t^\infty) = 1\}$. 

\begin{comment}
In fact, the following is likely true. \Alicomment{I think it easy to prove because $\psi_j(t)$-s are positively dependent. We don't use it in the rest of the proof but worth highlighting?}
\begin{fact}
    The random variables $\{\delta_{i,j}: i\in [n], j\in [m]\} \cup \{\psi_j(t^\infty)\}$ are positively dependent.
\end{fact}
\end{comment} 
That said, from the rearrangement inequality, we have
\begin{eqnarray}
&& \ex{\left.\prod_{i\in S_j^\downarrow} \left(1- \frac{\lambda_i}{1+\lambda_i}\cdot \exp\left(-\sum_{k\in N_i} \gamma_k \delta_{i,k}\right)   \right)\right| \psi_j(t^\infty) = 1} \nonumber\\
% &&\quad \leq \int_{0}^1 \prod_{i\in S_j^\downarrow} \left(1- \frac{\lambda_i}{1+\lambda_i}\cdot \exp\left(-\sum_{k\in N_i} \gamma_k F_{i,k}^{-1}(x)\right)   \right) dx  \ , 
&&\quad \leq \extwo{\tau_i \sim t_i}{\int_{0}^1 \prod_{i\in S_j^\downarrow} \left(1- \frac{\lambda_i}{1+\lambda_i}\cdot \exp\left(- F_{i}^{-1}(x,\tau_i)\right)   \right) dx } \ , \label{ineq:ubsm}
\end{eqnarray}
where $F_{i}(\cdot,\tau_i)$ is the CDF for the marginal distribution of $\sum_{k\in N_i} \gamma_k \delta_{i,k}$ conditional on $\psi_j(t^\infty) = 1$ and $t_i = \tau_i$.  By analyzing the correlation structure of these conditional distributions, we show that a constant-factor gap between $\sum_{k\in  N_i}\gamma_k\delta_{i,k}$ and $\sum_{k\in  N_i}\gamma_k\tau_i$ occurs with a constant probability.

\begin{lemma}\label{lem:main}
There exists constants $c, \bar{c}, \delta \in (0,1)$ such that for each $i \in S_j^\downarrow$, we have
\[ \pr{\left.\sum_{k\in  N_i}\gamma_k\delta_{i,k}\leq (1-c) \cdot t_i \sum_{k\in  N_i}\gamma_k  \right| t_i, \psi_j(t^\infty) =1} \geq \bar{c} \cdot {\bb I}[t_i \geq \tau_i^*] \ ,
\] where $\tau_i^* =  \frac{1}{\delta}\cdot \min\{\frac{1}{ \sum_{k \in N_i}{\gamma_k}/{\mu_i}},\frac{4}{1-\ln 2}\}$.
\end{lemma}

One implication of \Cref{lem:main} is that there exists a Bernoulli random variable $B_i$ with $\prpar{B_i = 1} = \prpar{B_i = 1 \; | \; (\delta_{i,k})_k, t_i} = \bar{c}$ (i.e., independent of $(\delta_{i,k})_k$ values and $t_i$) such that conditional on $\psi_j(t^\infty) = 1$, we have 
\begin{align}
\sum_{k \in N_i} {\gamma_k} \delta_{i,k} \stleq t_i \sum_{k \in N_i} \gamma_k - B_i \cdot {\bb I}[t_i \geq \tau_i^*] \cdot c \cdot t_i \sum_{k \in N_i} \gamma_k \ . \label{ineq:delta_dominated}
\end{align}


% \Alicomment{That's not the meaning of $B_i$ when we use it below. Below $B_i=1$ is the event in which $\sum_{k\in  N_i}\gamma_k\delta_{i,k}\leq (1-c) \sum_{k\in  N_i}\gamma_k\tau_i$. The statement would be the one below:}
% \Aliedit{That is, letting $B_i$ be a Bernoulli trial, independently drawn   with success probability $\pr{B_i = 1}=\pr{B_i = 1| t_i = \tau_i,\psi_j(t^\infty) =1} = 1-\bar{c}$, we have 
% \[ 
% \pr{\left. \sum_{k \in N_i} \gamma_k \delta_{i,k} \preceq_{st} B_i \left(\sum_{k\in N_i}\gamma_k \tau_i\right) + (1-B_i)\min\left\{\tau_i, (1-c)\max\{\tau_i,\tau^*_i\right\} \}\right| t_i = \tau_i,\psi_j(t^\infty) =1
% } = 1
%  \ .
% \]}


\Alicomment{Trying to give some intuition below, I am not sure if it is clear}
If there were no conditioning on $\psi_j(t^\infty) = 1$, the proof of Lemma~\ref{lem:main} would be relatively straightforward because there is a constant-factor gap in availability rates of offline vertices between sMc and vMc, which then translates into a gap between $\delta_{i,k}$-s and $\tau_i$. However, this gap in availability may not occur in the specific times where $j$ arrives (captured by the conditioning on $\psi_j(t^\infty) = 1$), e.g., due to bursts of arrivals. Proving Lemma~\ref{sec:lem:main} thus requires a fine-grained analysis of the correlation structure between $\delta_{i,k}$-s, which we develop in Section~\ref{sec:lem:main}. The crucial ingredients are bounds on the first-order and second-order moments of the cumulative duration of busy periods. Because the graph has a large degree, we essentially show that the mixing time of the queues is typically smaller than $\tau_i$, so the initial conditioning on $\psi_j(t^\infty) = 1$ washes away relatively quickly when we go backwards in time from $t^\infty$.
% Consider $T = \lceil\frac{1}{2}(1+e^{-\frac{1}{2}-\eps})^{-1}\tau_i (\sum_{j\in S_j}^+ \lambda_i)\rceil$ renewal cycles $\eta_j^-+\eta_j^+$. 
% By Bernstein's inequality for sub-exponential random variables, we infer that with high probability the sum of $T$ renewal times is smaller than $\tau_i$ but the sum of non-busy periods is larger than $\frac{e^{-\frac{1}{2}-\eps}}{2(1+e^{-\frac{1}{2}-\eps})}\tau_i$. Note that the sub-exponential condition is for $\alpha_{\max} = \max_{i\in S_j^\uparrow} (1+\sum_{k\in N_i} \gamma_k)^{-1} \leq 1$ and $(\nu^*)^2 = 2(1+e^{-\frac{1}{2}-\eps}) \frac{1}{\sum_{i\in S_j^\uparrow} \lambda_i}$.
% \end{proof}

% \Alicomment{Start with a  busy cycle and then use the fact that starting from a non-busy cycle is stochastically smaller than the steady state.}
% \begin{claim}
% For all $k\in [m]$, we have 
% \begin{eqnarray*}
% \expar{\delta_{i,k} |t_i = \tau_i,\psi_j(t^\infty) =1 } \leq \int_{0}^{\tau_i} e^{-\sum_{i\in S_j^+}\lambda_i x} \left(x+ (\tau_i-x)\cdot e^{-\frac{1}{2}+\eps} \right) dx \ .
% \end{eqnarray*}
% Therefore, there exists $\psi < 1$ such that for all $\tau_i\geq \frac{2}{\sum_{i\in S_j^\uparrow}\lambda_i}$,
% \begin{eqnarray*}
% \expar{\delta_{i,k} |t_i =\tau_i,\psi_j(t^\infty) =1 } \leq  \psi \tau_i\ .
% \end{eqnarray*}
% % \begin{eqnarray*}
% % \langle\delta_{i,k}  |t_i = \tau_i,\psi_j(t^\infty) =1 \rangle \succeq_{cxnd} Z + (\tau_i-Z)\cdot e^{-\frac{1}{2}-\eps}  \ .
% % \end{eqnarray*}
% \end{claim}
% Suppose $\tau_i\geq \frac{2}{\sum_{k\in N_i} \gamma_k}$. By Markov inequality, $\prpar{\sum_{k\in N_i} \gamma_k \delta_{i,k} \geq (1-\psi) \sum_{k\in N_i} \gamma_k\tau_i |t_i =\tau_i,\psi_j(t^\infty) =1} \leq  \frac{1-(1-e^{-0.5 c_1})\psi}{1-0.25 c_1\psi} <1$ where $\psi = (\frac{1}{4}(1+{(1+e^{-\frac{1}{2}-\eps})^{-1}})) $. Or by rearranging
% \begin{eqnarray} \label{ineq:markov}
% \pr{\sum_{k\in N_i} \gamma_k \delta_{i,k} < (1-0.25\psi) \sum_{k\in N_i} \gamma_k\tau_i} \geq  \frac{0.25-(1-e^{-0.5 c_1}) \psi}{1-0.25 c_1\psi} = c_2 >0 \ .
% \end{eqnarray}
% \Alicomment{TODO: Need to bounded away from $\tau_i = 0$}

The following result, which follows from the Hardy-Littlewood inequality (and rearrangement  inequality), intuitively says that the product of two random variables with fixed marginal distributions is maximized when they are perfectly positively associated:
\begin{fact}[c.f. \cite{burchard2006rearrangement}]\label{fact:rearrangement}
Let $X,Y \geq 0$ be two random variables with fixed marginal CDFs $F_X(\cdot)$ and $F_Y(\cdot)$, then we have $\expar{XY} \leq \int_{0}^1 F_X^{-1}(u)\cdot F_Y^{-1}(u)  du$.
\end{fact}

\paragraph{Proof of the theorem.}
\begin{align}
    &\ex{\left.\prod_{i\in S_j^\downarrow} \left(1- \frac{\lambda_i}{\mu_i+\lambda_i}\cdot \exp\left(-\sum_{k\in N_i} \gamma_k \delta_{i,k}\right)   \right)\right| \psi_j(t^\infty) = 1} \nonumber \\ & \quad \overset{(1)}{\leq}  \extwo{(\tau_i \sim t_i)_{i}}{\int_{0}^1\prod_{i\in S_j^\downarrow} \left(1- \frac{\lambda_i}{\mu_i+\lambda_i}\cdot \exp\left(- F_{i}^{-1}(u,\tau_i)\right)   \right) du } \nonumber \\ & \quad \overset{(2)}{\leq}  \extwo{(\tau_i \sim t_i)_{i}}{\int_{0}^1\prod_{i\in S_j^\downarrow} \left(1- \frac{\lambda_i}{\mu_i+\lambda_i}\cdot \exp\left(- \tilde{F}_{i}^{-1}(u,\tau_i)\right)   \right) du } \nonumber \\ & \quad \overset{(3)}{=} (1-\bar{c})\cdot \ex{\prod_{i\in  S_j^\downarrow} \left( 1- \frac{\lambda_i}{\mu_i+\lambda_i}\cdot \exp\left(-t_i \sum_{k\in N_i} \gamma_k \right)\right)} \nonumber \\ & \quad \quad + \bar{c} \cdot \ex{\prod_{i\in  S_j^\downarrow} \left( 1- \frac{\lambda_i}{\mu_i+\lambda_i}\cdot \exp\left(-\left(1- c \cdot {\bb I}\left[t_i \geq \tau_i^*\right]\right) \cdot t_i \sum_{k \in N_i} \gamma_k \right)\right)}\nonumber \\ & \quad \overset{(4)}{=} (1-\bar{c})\cdot \ex{\prod_{i\in  S_j^\downarrow} \left( 1- \frac{\lambda_i}{\mu_i+\lambda_i}\cdot \exp\left(-t_i \sum_{k\in N_i} \gamma_k \right)\right)} \nonumber \\ & \quad \quad + \bar{c} \cdot \prod_{i\in  S_j^\downarrow} \left(1- \frac{\lambda_i}{\mu_i + \lambda_i+ (1-c') \sum_{k\in N_i} \gamma_k }\right) \ , \label{ineq:final_close} 
\end{align}
where (1) follows from \Cref{fact:rearrangement} and $F_i(\cdot, \tau_i)$ is the conditional CDF of $\sum_{k \in N_i} \gamma_k \delta_{i,k}$ given $t_i = \tau_i$ for every $1 \leq i \leq |S_j^\downarrow|$. In (2), $\tilde{F}_i(\cdot, \tau_i)$ is a two-point distribution corresponding to the RHS of inequality \eqref{ineq:delta_dominated} i.e., it is the conditional CDF of $t_i \sum_{k \in N_i} \gamma_k - B_i \cdot {\bb I}[t_i \geq \tau_i^*] \cdot c \cdot t_i \sum_{k \in N_i} \gamma_k$ given $t_i = \tau_i$. Thus, step (2) uses inequality \eqref{ineq:delta_dominated} from \Cref{lem:main} which posits that for every fixed value of $u$ and $\tau_i$, we have $F_i(u, \tau_i) \leq \tilde{F}_i(u, \tau_i)$. Consequently, step (3) again uses \Cref{fact:rearrangement} by noting that the LHS of the equality corresponds to random variables $(B_i)_i$ that are perfectly positively associated. Since these are Bernoulli random variables with the same parameter, the perfect positive association happens when they are all equal, as apparent from the RHS of step (3). Lastly, (4) follows from the following observation:
\begin{align}
    & \ex{\exp\left(-\left(1- c \cdot {\bb I}\left[t_i \geq \tau_i^*\right]\right) \cdot t_i \sum_{k \in N_i} \gamma_k \right)} \nonumber \\ & \quad = \int_{0}^\infty (\mu_i+\lambda_i)\exp(-(\mu_i+\lambda_i)\tau) \cdot \exp\left(-\left(1- c \cdot {\bb I}\left[\tau \geq \tau_i^*\right]\right) \cdot \tau \sum_{k \in N_i} \gamma_k \right) d \tau  \nonumber \\ & \quad = \int_{0}^{\tau_i^*} (\mu_i+\lambda_i)\exp(-(\mu_i+\lambda_i)\tau) \cdot \exp\left(-\tau \sum_{k \in N_i} \gamma_k \right) d \tau  \nonumber \\ & \quad \quad + \int_{\tau_i^*}^\infty (\mu_i+\lambda_i)\exp(-(\mu_i+\lambda_i)\tau) \cdot \exp\left(-\left(1-c\right) \tau \sum_{k \in N_i} \gamma_k \right) d \tau  \nonumber \\ & \quad = \frac{(\mu_i+\lambda_i) \cdot \left(1 - e^{-\left(\mu_i+\lambda_i + \sum_{k \in N_i} \gamma_k \right)\tau_i^*}\right) }{\mu_i+\lambda_i + \sum_{k \in N_i} \gamma_k}  + \frac{(\mu_i+\lambda_i)e^{-\left(\mu_i + \lambda_i + (1-c)\sum_{k \in N_i} \gamma_k \right)\tau_i^*}}{\mu_i + \lambda_i + (1-c)\sum_{k \in N_i} \gamma_k} \notag \\ & \quad \geq \frac{(\mu_i+\lambda_i) \cdot \left(1 - e^{-\left(\mu_i+\lambda_i + \sum_{k \in N_i} \gamma_k \right)\tau_i^*}\right) }{\mu_i+\lambda_i + \sum_{k \in N_i} \gamma_k}  + \frac{(\mu_i+\lambda_i)e^{-\left(\mu_i + \lambda_i + \sum_{k \in N_i} \gamma_k \right)\tau_i^*}}{\mu_i + \lambda_i + (1-c)\sum_{k \in N_i} \gamma_k} \notag  \\ & \quad \geq  \frac{\mu_i + \lambda_i}{\mu_i+\lambda_i+ (1-c')\sum_{k\in N_i} \gamma_k} \ ,  \label{ineq:offline_avl_surplus}
\end{align}
where $c' = c e^{-(\mu_i+\lambda_i+ \sum_{k\in N_i} \gamma_k)\tau_i^*}\geq ce^{-\frac{1}{\delta}[(1+\eps^2)4(1-\ln 2)^{-1} + 1] }$ is obtained from the Jensen's inequality with function $x \to \frac{\mu_i+\lambda_i}{\mu_i + \lambda_i + (1-x) \sum_{k \in N_i} \gamma_k}$. 

We now explain how the bound in \eqref{ineq:final_close} translates to a constant factor boost in the availability probability of offline vertices. Intuitively, the boost in availability probability in \eqref{ineq:offline_avl_surplus} is influential only if $\Gamma_i := \sum_{k \in N_i} \gamma_k$ is large. Therefore, define $I^+\subseteq S_j^\downarrow$ as the subset of offline vertex types $i$ such that $\Gamma_i \geq \delta'$, where $\delta' > 0$ is a constant that we specify later. Inequality \eqref{ineq:abandonment_bound} and the property of $j$-balancedness imply that 
\[
\sum_{i\in S_j^\downarrow\setminus I^+} \lambda_i \leq (1+\delta') \sum_{i\in S_j^\downarrow\setminus I^+} x_{i,a}   \leq (1+\delta')\left(\frac{1}{2}+\eps\right) \leq \frac{1}{2} + 2\delta'+\eps\ .
\]
In turn, our tightening constraints and inequality \eqref{ineq:abandonment_bound} imply that 
\[
\sum_{i\in S_j^\downarrow\setminus I^+} x_{i,a} \leq \frac{1}{1-\eps} \cdot \sum_{i\in S_j^\downarrow\setminus I^+} \frac{1}{\gamma_j} x_{i,j} \leq \frac{1}{1-\eps} \cdot \left(1-e^{-(\frac{1}{2} + 2\delta'+\eps)}\right) \ .
\]
Consequently, 
\[
\frac{1}{1-\eps} \cdot \sum_{i\in I^+} \frac{\lambda_i}{1+\sum_{k\in N_i} \gamma_k } \geq \sum_{i \in I^+} x_{i,a} = \sum_{i\in  S_j^\downarrow} x_{i,a} - \sum_{i\in  S_j^\downarrow\setminus I^+} x_{i,a}   \geq e^{-(\frac{1}{2}+4 \delta'+ 2\eps)} - \frac{1}{2}-\eps \ .
\]
This yields
\begin{eqnarray} \label{ineq:density}
  1\geq \sum_{i\in I^+} \frac{\lambda_i}{1+\lambda_i+\sum_{k\in N_i} \gamma_k } = \sum_{i\in  S_j^\downarrow} x_{i,a} - \sum_{i\in  S_j^\downarrow\setminus I^+} x_{i,a}   \geq e^{-(\frac{1}{2}+4 \delta'+ 2\eps)} - \frac{1}{2}-\eps - \eps^2  = \kappa(\eps,\delta') \ .
\end{eqnarray}
Choosing $\delta' = \frac{1}{8}$ ensures that $\kappa(\eps,\delta')>\kappa'>0$ for sufficiently small $\eps$.

\paragraph{Stochastic dominance.} 



Let us revert to the upper bound in~\eqref{ineq:ubsm}, which we restate as follows:
\begin{eqnarray}
&& \ex{\left.\prod_{i\in S_j^\downarrow} \left(1- \frac{\lambda_i}{1+\lambda_i}\cdot \exp\left(-\sum_{k\in N_i} \gamma_k \delta_{i,k}\right)   \right)\right| \psi_j(t^\infty) = 1} \nonumber\\
&&\quad \leq \extwo{\tau_i \sim t_i}{\int_{0}^1\prod_{i\in S_j^\downarrow} \left(1- \frac{\lambda_i}{1+\lambda_i}\cdot \exp\left(- F_{i}^{-1}(u,\tau_i)\right)   \right) du } \nonumber\\
&&\quad \leq \extwo{\tau_i \sim t_i}{\int_0^1\prod_{i\in S_j^\downarrow} \left(1- \frac{\lambda_i}{1+\lambda_i}\cdot \exp\left(- \tilde{F}_{i}^{-1}(u,\tau_i)\right)   \right) du}\nonumber\\
&&= (1-\bar{c})\cdot \ex{\prod_{i\in  S_j^\downarrow} \left( 1- \frac{\lambda_i}{1+\lambda_i}\cdot \exp\left(-\sum_{k\in N_i} \gamma_k t_i\right)\right)} \nonumber\\
&& \qquad + \bar{c} \ \ex{\prod_{i\in  S_j^\downarrow} \left( 1- \frac{\lambda_i}{1+\lambda_i}\cdot \exp\left(-\sum_{k\in N_i} \gamma_k \min\{t_i, (1-c)\max\{t_i,\tau^*_i\}\}\right)\right)}\nonumber\\
&&\approx (1-\bar{c})\cdot \frac{1}{e} \exp\left(\sum_{i\in S_j^\uparrow} x_{i,a}\right) \nonumber\\
&& \qquad + \bar{c} \prod_{i\in  S_j^\downarrow} \left(1- \frac{\lambda_i}{1+\lambda_i}\cdot \ex{\exp\left(-\sum_{k\in N_i} \gamma_k \min\{t_i, (1-c)\max\{t_i,\tau^*_i\}\}\right)}\right)\\
&&\leq (1-\bar{c})\cdot \frac{1}{e} \exp\left(\sum_{i\in S_j^\uparrow} x_{i,a}\right) \nonumber\\
&& \qquad + \bar{c} \prod_{i\in  S_j^\downarrow} \left(1- \frac{\lambda_i}{1+\lambda_i+\sum_{k\in N_i} \gamma_k (1-c')}\right)\ , \label{ineq:final_close}
\end{eqnarray} 
where we define $\tilde{F}(\cdot,\tau_i)$ as two-point distribution $B_i(\sum_{k\in N_i}\gamma_k \tau_i) + (1-B_i)\min\{\tau_i, (1-c)\max\{\tau_i,\tau^*_i\}\}$, with $B_i$ a Bernoulli random variable with success rate $\prpar{B_i =1}  =1 - \bar{c}$ ($\bar{c}$ being the constant in Lemma~\ref{lem:main})  and $\tau^*_i = \frac{1}{\delta}\cdot \min\{\frac{1}{ \sum_{k\in N_i}\gamma_k},\frac{4}{1-\ln 2}\}$. The second inequality proceeds from Lemma~\ref{lem:main}. Indeed, we can restate that lemma as $\sum_{k\in N_i}\gamma_k \delta_{i,k} \preceq B_i(\sum_{k\in N_i}\gamma_k t_i) + (1-B_i)\min\{t_i, (1-c)\max\{t_i,\tau^*_i\}\}$ after we condition on $t_i = \tau_i$ and $\psi_j(t^\infty)=1$. In the last inequality, $c'$ is a universal constant obtained from
\begin{eqnarray*}
&&\ex{\exp\left(-\sum_{k\in N_i} \gamma_k \min\{t_i, (1-c)\max\{t_i,\tau^*_i\}\}\right)} \\
&&\quad= \int_{0}^{+\infty} (1+\lambda_i)e^{- (1+\lambda_i)t-\sum_{k\in N_i} \gamma_k \min\{t_i, (1-c)\max\{t_i,\tau^*_i\}\} } dt \\
&&\quad \geq  \int_{0}^{\tau_i^*} (1+\lambda_i)e^{- (1+\lambda_i)t-\sum_{k\in N_i} \gamma_k  t} dt + \int_{\tau_i^*}^{+\infty} (1+\lambda_i)e^{-(1+\lambda_i)t-\sum_{k\in N_i} (1-c)\gamma_kt  } dt\\
&&\quad =  \frac{1+\lambda_i}{1+\lambda_i+ \sum_{k\in N_i} \gamma_k}\left[1-e^{-(1+\lambda_i+ \sum_{k\in N_i} \gamma_k)\tau_i^*}\right] + \frac{1+\lambda_i}{1+\lambda_i+ \sum_{k\in N_i} (1-c)\gamma_k}\left[e^{-(1+\lambda_i+ \sum_{k\in N_i} \gamma_k)(1-c)\tau_i^*}\right]\\
&&\quad \geq  \frac{1+\lambda_i}{1+\lambda_i+ (1-c')\sum_{k\in N_i} \gamma_k}
\end{eqnarray*}
where the last inequality follows from Jensen's with $c' = c e^{-(1+\lambda_i+ \sum_{k\in N_i} \gamma_k)(1-c)\tau_i^*}\geq ce^{-\frac{1}{\delta}[(1+\eps^2)4(1-\ln 2)^{-1} + 1] }   $.

Define $I^+\subseteq S_j^\downarrow$ as the subset of offline vertex types $i$ such that $\sum_{k\in N_i} \gamma_k / \mu_i \geq \delta'$.  The property of $j$-balancedness implies that 
\[
\sum_{i\in S_j^\downarrow \setminus I^+} \lambda_i \leq (1+2 \delta') \sum_{i\in S_j^\downarrow\setminus I^+} x_{i,a}   \leq (1+2 \delta')\left(\frac{1}{2}+\eps\right) =\frac{1}{2} + 4\delta'+2\eps\ .
\]
In turn, our tightening constraints imply that 
\[
\sum_{i\in S_j^\downarrow\setminus I^+} x_{i,a} \leq (1+\eps) \sum_{i\in S_j^\downarrow\setminus I^+} \frac{1}{\gamma_j} x_{i,j} \leq 1-e^{-(\frac{1}{2}+4\delta' + 2\eps)}\ .
\]
Consequently,
\[
\sum_{i\in I^+} \frac{\lambda_i}{1+\sum_{k\in N_i} \gamma_k } = \sum_{i\in  S_j^\downarrow} x_{i,a} - \sum_{i\in  S_j^\downarrow\setminus I^+} x_{i,a}   \geq e^{-(\frac{1}{2}+4 \delta'+ 2\eps)} - \frac{1}{2}-\eps \ .
\]
This yields
\begin{eqnarray} \label{ineq:density}
  1\geq \sum_{i\in I^+} \frac{\lambda_i}{1+\lambda_i+\sum_{k\in N_i} \gamma_k } = \sum_{i\in  S_j^\downarrow} x_{i,a} - \sum_{i\in  S_j^\downarrow\setminus I^+} x_{i,a}   \geq e^{-(\frac{1}{2}+4 \delta'+ 2\eps)} - \frac{1}{2}-\eps - \eps^2  = \kappa(\eps,\delta') \ .
\end{eqnarray}
Choosing $\delta' = \frac{1}{8}$ ensures that $\kappa(\eps,\delta')>\kappa'>0$ for sufficiently small $\eps$. To conclude, we observe that there exists a constant $c''>1$ such that, for sufficiently small $\eps$:
\begin{eqnarray*}
\prod_{i\in  I^+} \left(1- \frac{\lambda_i}{1+\lambda_i+\sum_{k\in N_i} \gamma_k (1-c')}\right) & \leq & \prod_{i\in  I^+} \exp\left(- \frac{\lambda_i}{1+\lambda_i+\sum_{k\in N_i} \gamma_k (1-c')}\right)\\
& \leq &  \exp\left(-\sum_{i\in  I^+}\frac{1+\eps^2+\delta'}{1+\eps^2 + (1-c')\delta'}\cdot \frac{\lambda_i}{1+\lambda_i+\sum_{k\in N_i} \gamma_k }\right)\\
& \leq &  \left(1-\frac{c' \dot \kappa'}{e(8+8\eps^2 + (1-c'))}\right)\exp\left(- \sum_{i\in  I^+} \frac{\lambda_i}{1+\lambda_i+\sum_{k\in N_i} \gamma_k }\right)\\
& \leq &  \frac{1}{c''}\exp\left(- \sum_{i\in  I^+} \frac{\lambda_i}{1+\lambda_i+\sum_{k\in N_i} \gamma_k }\right)\ ,
% &\approx &\frac{1}{c''} \prod_{i\in  I^+} \left(1- \frac{\lambda_i}{1+\lambda_i+\sum_{k\in N_i} \gamma_k }\right) \ ,
\end{eqnarray*}
where the second inequality holds since $\sum_{k\in N_i} \gamma_k\geq \delta'$ for every $i\in I^+$ and th third inequality follows from~\eqref{ineq:density}.
Plugging this inequality into~\eqref{ineq:final_close} yields the desired result.
% This leads to the robust optimization problem
% \begin{eqnarray*}
% \max_{G_i} && \extwo{U\sim [0,1]}{\prod_{i\in S_j^\downarrow} \left(1- \frac{\lambda_i}{1+\lambda_i}\cdot \exp\left(- G_{i}^{-1}(U,\tau_i)\right)   \right) }\\
% &s.t.&\\
% &&\qquad \extwo{g\sim G_i(\cdot,\tau_i)}{ 1- \frac{\lambda_i}{1+\lambda_i} e^{-g}} \leq 1- \frac{\lambda_i}{1+\lambda_i} e^{- c^{-1}\cdot\sum_{k\in N_i} \gamma_k \tau_i} \qquad \forall i \in S_j^\downarrow \\
% &&\qquad G^{-1}_i(1,\tau_i) \leq  \sum_{k\in N_i} \gamma_k \tau_i \qquad \forall i \in S_j^\downarrow
% \end{eqnarray*}

% \paragraph{Case 5: Some of $j$'s contributions from offline nodes are concentrated on one $i$.}
% \begin{obs}
% Suppose  that $\sum_{i \in S_j} \frac{x_{i,j}}{\gamma_j} \ge 1 - \epsilon$ and $P_{i,j}\geq (1-\eps)$ for all $i\in S_j$. Moreover, there exists  $i^* \in S_j$ $\frac{x_{i^*,j}}{\gamma_j} \geq (1-\eps)\frac{x_{i^*,a}}{\mu_{i^*}} \geq \eps $. Then, we have $\textup{\textsf{ALG}}_j \geq (1-1/e+c(\epsilon)) \cdot \textsf{LP}_{\{j\}}$ for some constant $c(\eps)$ that only depends on $\eps$.
% \end{obs}
% \begin{proof}
% Denote by ${R}^-_j(1)$ the number of proposal requests to $j$ from offline vertices other than $i$. Then, we have
% \begin{eqnarray*}
% \mathbb{E}[\min(1, R_j(1))] 
%     &= & \left(1-\exp\left(-\frac{x_{i^*,a}}{\mu_{i^*}}\right)\right) + \exp\left(-\frac{x_{i^*,a}}{\mu_{i^*}}\right)\mathbb{E}[\min(1, R^-_j(1))] \\
%     &= & \left(1-\exp\left(-\frac{x_{i^*,a}}{\mu_{i^*}}\right)\right) + \exp\left(-\frac{x_{i^*,a}}{\mu_{i^*}}\right)\mathbb{E}[\min(1, R^-_j(1))] \\
%     &= & \left(1-\exp\left(-\frac{x_{i^*,a}}{\mu_{i^*}}\right)\right) + \exp\left(-\frac{x_{i^*,a}}{\mu_{i^*}}\right)\mathbb{E}\left[\min\left(1, \text{Pois}\left(\sum_{i\in S_j \setminus \{i^*\}} x_{i,j}/\gamma_j\right)\right)\right] \\
%     &= & \left(1-\exp\left(-\frac{x_{i^*,a}}{\mu_{i^*}}\right)\right) + \exp\left(-\frac{x_{i^*,a}}{\mu_{i^*}}\right)\left(1-\exp\left(-\sum_{i\in S_j \setminus \{i^*\}} x_{i,j}/\gamma_j\right)\right) \\
%     &= & \left(1-\exp\left(-\frac{x_{i^*,a}}{\mu_{i^*}}\right)\right) + \exp\left(-\frac{x_{i^*,a}}{\mu_{i^*}}\right)\left(1-\exp\left(-\max\left\{0,(1-\eps) +\frac{x_{i^*,a}}{\mu_{i^*}}\right\} \right)\right) \\
% \end{eqnarray*}
    
% \end{proof}

%Let  $\textsf{LP}_j(w) := \sum_{i : r_{i,j} \ge w} \frac{x_{i,j}}{\gamma_j} \cdot r_{i,j}$. Say there exists some $w$ such that $\textsf{LP}_j(w) \ge (1-\epsilon) \cdot \textsf{LP}_j(0)$ and $\sum_{i : r_{i,j} \ge w} \frac{x_{i,j}}{\gamma_j} \le 1 - \epsilon$. Then, 



% \Alirezaedit{For $T \subseteq I$ and $S \subseteq J$, let $\textsf{LP}_{S,T} = \sum_{i \in T} \sum_{j \in S} \frac{x_{i,j}}{\gamma_j}$. 
  
\subsubsection{Proof of Lemma~\ref{lem:main}}
 \label{sec:lem:main}
Note that the proportion of time spent in a blocked cycle $\psi_j(t)=1$ is equal to $\prpartwo{s}{\psi_j(t)=1} \leq e^{-\frac{1}{2}+\eps}$ from inequality~\eqref{ineq:balanced}. From renewal theory, this is also equal to $\frac{\expar{\eta^+_{j}}}{\expar{\eta^+_{j}+\eta^-_{j}}}$ where $\eta^+_{j},\eta^-_{j}$ are the random durations for one busy cycle and one non-busy cycle, respectively. Since $\expar{\eta^+_{j}} = \frac{1}{\sum_{i\in S_j^\uparrow}\lambda_i}$, we obtain 
\begin{eqnarray}
\expar{\eta^{-}_j} \geq \frac{1 -  e^{-\frac{1}{2}+\eps}}{ e^{-\frac{1}{2}+\eps}} \cdot \frac{1}{\sum_{i\in S_j^\uparrow}\lambda_i} \ .
\end{eqnarray}
% I believe that this inequality implies the following. 
The following claim offers bounds on the first-order and second-order moments of the busy periods.
\begin{claim} \label{clm:nonbusy}
Let $I \subseteq [n]$ be a subset of offline vertices and consider their blocked and non-blocked cycles $\eta_1^+, \eta_1^-, \ldots$ under the vMc (i.e., during $\eta_t^+$, we have $\sum_{i \in I} Q_i^v = 0$). Then, assuming we start at a blocked cycle, all the cycles of a type (i.e., blocked or non-blocked) are i.i.d. and $\eta_{1}^-$ stochastically dominates a hyperexponential distribution $Z = \sum_{i\in I} \frac{\lambda_i}{\sum_{i'\in I} \lambda_{i'}} \cdot Exp(\mu_i + \sum_{k \in N_i}\gamma_k)$ with 
\begin{eqnarray*}
    \ex{Z} = \frac{1}{\sum_{i\in I} \lambda_i}\sum_{i \in I}  \frac{\lambda_i}{\mu_i + \Gamma_i} \geq (1-\eps) \sum_{i \in I} \frac{x_{i,a}}{\mu_i} \cdot \frac{1}{\sum_{i \in I} \lambda_i}
\end{eqnarray*}
and 
\begin{eqnarray*}
    \Var[Z] \leq \ex{Z^2} = \frac{2}{\sum_{i \in I} \lambda_i}\sum_{i\in I}  \frac{\lambda_i}{(\mu_i + \Gamma_i)^2} \leq \frac{2}{\min_{i \in I} (\mu_i + \Gamma_i)} \cdot \ex{Z}\ .
\end{eqnarray*}
\end{claim}
\begin{proof}
A non-blocked cycle starts with randomly drawing a type $i \in I$ with probability $\frac{\lambda_i}{\sum_{i' \in I} \lambda_{i'}}$ and it cannot end until that vertex leaves after an Exponentially-distributed duration $Exp(\mu_i + \Gamma_i)$. The claim straightforwardly follows from applying inequality \eqref{ineq:abandonment_bound}. 
\end{proof}

% \Alicomment{Now I need to revist the next claim to get a bound on first-order and second-order moment}


Define $J^{\rm indep} = \{k\in B: \sum_{i\in S_k^\uparrow\setminus S_j^\uparrow} x_{i,a} \geq \kappa_1\delta \}$ and $J^{\rm correl} = \{k\in B: \sum_{i\in S_k^\uparrow\cap S_j^\uparrow} x_{i,a} \geq (1-\epsilon)/2 -\kappa_1\delta\}$, where $\kappa_1$ is a large constant we choose later.\footnote{Note that $j$ was fixed throughout the proof, so we omit the index in defining $J^{\rm indep}$ and  $J^{\rm correl} $.} These sets partition the online vertices $B= J^{\rm indep}\sqcup J^{\rm correl}$ from balancedness. 


% Observe that for every $i\in S_j^\downarrow$
% \begin{eqnarray} \label{ineq:difficult_type1}
%     \sum_{k\in J^{\rm correl} } \gamma_k \leq (1+\eps)\sum_{k\in J^{\rm correl}}\sum_{i\in S_k} x_{i,k} \leq 2(1+2\eps+2\kappa_1\delta)\sum_{k\in J^{\rm correl}}\sum_{i\in S_k^\uparrow \cap S_j^\uparrow} x_{i,k} \leq 2(1+2\eps+2\kappa_1\delta) \sum_{i\in S_j^\uparrow} \lambda_i\ .
% \end{eqnarray}
%  Moreover, balancedness implies that for each $i\in S_j^\downarrow$
% \begin{eqnarray} \label{ineq:difficult_type2}
% \sum_{\alpha\in S_j^\uparrow}\frac{\lambda_\alpha}{\sum_{b\in S_j^\uparrow}\lambda_b} \frac{\sum_{k\in J^{\rm correl} \cap N_i} \gamma_k {\bb I} [\alpha\in S_k^\uparrow]}{1+\sum_{k \in N_\alpha} \gamma_k}&=&\sum_{\alpha\in S_j^\uparrow}\frac{x_{\alpha,a}}{\sum_{b\in S_j^\uparrow}\lambda_b} {\sum_{k\in J^{\rm correl} \cap N_i} \gamma_k {\bb I} [a\in S_k^\uparrow]} \nonumber\\
% &=&\frac{1}{\sum_{b\in S_j^\uparrow}\lambda_b} \sum_{k\in J^{\rm correl} \cap N_i} \gamma_k \left(\sum_{\alpha\in S_j^\uparrow \cap S_k^\uparrow }{x_{\alpha,a}}\right)\nonumber\\
% & \geq & \left(\frac{1}{2}-\eps-\kappa_1\delta\right)\frac{\sum_{k\in J^{\rm correl}\cap N_i} \gamma_k}{\sum_{b\in S_j^\uparrow}\lambda_b}  \ .
% \end{eqnarray}

\begin{lemma} \label{lem:correl}
There exist constants $c_0, c_1 \in (0,1)$ such that for each $i \in S_j^\downarrow$, we have 
\[ \pr{\left.\sum_{k\in J^{\rm correl}\cap N_i}\gamma_k\delta_{i,k}\leq (1-c_0) \cdot t_i \sum_{k\in J^{\rm correl}\cap N_i}\gamma_k  \right| t_i, \psi_j(t^\infty) =1} {\geq} c_1 \cdot {\bb I}[t_i \geq \tilde{\tau}_i] \ ,
\] where $\tilde{\tau}_i = \frac{1}{\delta}\cdot \min\{\frac{1}{\sum_{k\in J^{\rm correl}\cap N_i}\gamma_k},\frac{4}{1-\ln 2}\}$. 

\end{lemma}
\begin{proof}
To simplify notation, we make the conditioning on $\{\psi_j(t^\infty) =1\}$ implicit throughout this proof and assume that $t_i \geq \tilde{\tau}_i$.
To analyze the cumulative blocked and non-blocked times, we make use of tail bounds. Recall that, for $Y$ being a sum of $n$ i.i.d. exponential random variables, we have~\cite[Thm.~5.1]{janson2018tail} for all $\lambda\geq 1$
\begin{eqnarray} \label{ineq:expconcentration}
\pr{Y\geq \lambda \ex{Y}} \leq \frac{1}{\lambda}e^{-n(\lambda-1-\ln(\lambda))} \ .
\end{eqnarray}
We will also make use of Paley–Zygmund inequality for $Y\geq 0$,
\begin{eqnarray} \label{ineq:hyperconcentration}
\pr{Z\geq \theta \ex{Z}} \geq (1-\theta)^2\frac{\expar{Z}^2}{\ex{Z^2}} \ .
\end{eqnarray}

\paragraph{Existence of core set of offline vertices.} We prove that the subgraph induced by $S^\downarrow_j$ and $J^{\rm correl} \cap N_i$ is highly connected.
\begin{claim} \label{fact:1core}
Suppose that sets $S_1,\ldots,S_K\subseteq[N]$ satisfy $|S_k| \geq (1-\eps)N$ for all $k\in [K]$. Then, for all $\theta\in (0,1-\eps)$ there exist $S^*\subseteq [N]$ such that  $|S^*| \geq \frac{1-\theta-\eps}{1-\theta}N$ and for each $i\in S^*$, $|\{k\in [K]: i\in S_k\}| \geq \theta K$.
\end{claim}
\begin{proof}
Order $i\in [N]$ by decreasing $c_i = \sum_{k\in [K]} {\bb I}[i\in S_k]$. Consider $i_0 = \max\{i\in [0,N]: c_i \geq \theta K \}$. Then, $\sum_{i\leq i_0} c_i \leq i_0 K$. At the same time, $\sum_{i\leq i_0} c_i \geq (1-\eps)NK - (N-i_0)\cdot\theta K = (1-\theta-\eps)NK + i_0\theta K$. This implies that $i_0 \geq \frac{1-\theta-\eps}{1-\theta}N$. 
\end{proof}
This leads to a generalization of the union bound:
\begin{claim}\label{fact:2core}
Suppose that events $E_1,\ldots E_K$ with weights $\tilde{\gamma}_1,\ldots,\tilde{\gamma}_K$ satisfy $\prpar{E_k}\geq 1-\eps$ for all $k\in [K]$. Then, there exists $E^*$ with $\prpar{E^*}\geq 1-2\eps$ such that $\prpar{\sum_{k=1}^K \tilde{\gamma}_k {\bb I}[E_k] \geq \frac{1}{2}\sum_{k=1}^K \tilde{\gamma}_k|E^*} = 1$.
\end{claim}
\begin{proof}
Interpret each event $E_k$ as a corresponding subset of realizations $S_k$ for the empirical  measure on discrete outcomes. Duplicate each subset $S_k$ exactly $\lceil K\frac{\tilde{\gamma}_{k}}{\sum_{k'} \tilde{\gamma}_{k'}} \rceil$ times for a very large $K$. Apply Claim~\ref{fact:1core} with $\theta=1/2$.
\end{proof}

Now, fix any $i\in S_j^\downarrow$. We use the following analogy. Take the ground set $\Omega = S^\uparrow_j$ and use the probability measure $\prpar{\alpha} = \frac{x_{\alpha,a}}{\sum_{\beta\in \Omega}x_{\beta,a}}$. Define $[K]= J^{\rm correl} \cap N_i$, the events $E_k = S^\uparrow_j\cap S^\uparrow_k$, and the weights $\tilde{\Gamma}_k = \gamma_k$. By the definition of Correl types and $j$-balancedness, for every $k\in [K]$
\begin{eqnarray}
\pr{E_k} = \sum_{\alpha\in S^\uparrow_j\cap S^\uparrow_k} \frac{x_{\alpha,a}}{\sum_{\beta\in S^\uparrow_j}x_{\alpha,a}} \geq \frac{\frac{1}{2} - \eps -\kappa\delta}{\frac{1}{2}+\eps} \geq 1- 3\eps - 2\kappa\delta \ .
\end{eqnarray}
Now, Claim~\ref{fact:2core} implies that there exists a subset $I^{\rm core}\subseteq S_j^{\uparrow}$ such that 
\begin{eqnarray}\label{ineq:core}
 \sum_{\alpha\in I^{\rm core}} x_{\alpha, a} \geq \frac{1}{2} - 4 \eps -2 \kappa 
\delta   
\end{eqnarray}
and, for each $\alpha\in I^{\rm core}$,  
\begin{eqnarray} \label{prop:core}
\sum_{k\in J^{\rm correl} \cap N_i} \gamma_k {\bb I}[\alpha\in S^\uparrow_k] \geq \frac{1}{2}\sum_{k\in J^{\rm correl} \cap N_i} \gamma_k \ .
\end{eqnarray}
In particular, we also infer that 

\begin{eqnarray} \label{ineq:subsume}
&&\sum_{\alpha\in I^{\rm core}} \lambda_\alpha \geq \sum_{\alpha\in I^{\rm core}} \sum_{k\in J^{\rm correl} \cap N_i} x_{\alpha,k} = \sum_{\alpha\in I^{\rm core}} \sum_{k\in J^{\rm correl} \cap N_i} x_{\alpha,a}\gamma_k {\bb I}[\alpha\in S^\uparrow_k]  \nonumber \\
&&\qquad\geq \frac{1}{2} \left(\sum_{\alpha\in I^{\rm core}} x_{\alpha,a}\right) \cdot \left(\sum_{k\in J^{\rm correl} \cap N_i} \gamma_k\right) \geq \left(\frac{1}{4} - 2 \eps - \kappa \right) \cdot \left(\sum_{k\in J^{\rm correl} \cap N_i} \gamma_k\right) \ .
\end{eqnarray}

% Let $M>0$ be a constant we tune later. \Alicomment{We will likely choose $M=\frac{1}{2}\log\frac{1}{\delta}$. Now I think $M=2$. It turns out $M=\frac{4}{(1-\ln 2)}$}
\paragraph{Case 1: $\boldsymbol{{\sum_{k\in J^{\rm correl}\cap N_i}\gamma_k}\geq \frac{4}{(1-\ln 2)}}$.} To ease the notation, let $\tilde{\Gamma} = \sum_{k\in J^{\rm correl}\cap N_i}\gamma_k$ and $\tilde{\Lambda} = \sum_{i' \in I^{\rm core}} \lambda_{i'}$. In this case, we use a narrower definition of a blocked period as a time $t$ where we require $\sum_{i' \in I^{\rm core}} Q_{i'}(t) = 0$. Other times are said to be non-blocked periods. Consider $T = \lceil (\tilde{\Lambda}/(\delta' \tilde{\Gamma})\rceil$ blocked and non-blocked cycles, which we respectively denote by $\eta^+_1,\eta^-_1,\ldots,\eta^+_T,\eta^-_T$. Here, $\delta' \leq 4\delta$ is an auxiliary parameter that we specify later. Inequality \eqref{ineq:subsume} gives $T \geq \frac{1/4 - 2\eps - \kappa}{\delta'}$. From the time-reversibility of the top vMc queues, we go backward in time from $t^\infty$, starting initially from a busy cycle. The cycles from each type are i.i.d. with $\eta^+_1\sim Exp(\tilde{\Lambda})$ and $\eta^-_1 \succeq Z$ from Claim~\ref{clm:nonbusy}. Here, we note that $Z$ hyperexponential distribution formed by the mixture $\{p_{i'}\}_{i' \in I^{\rm core}}$ with $p_{i'} = {\lambda_{i'}}/{\tilde{\Lambda}}$ of exponential distributions $Exp(1 +\sum_{k\in  N_{i'}} \gamma_k)$. In particular, inequality~\eqref{ineq:core} and $j$-balancedness imply that 
\begin{align}\label{ineq:z_bounds}
    \ex{Z} \geq (1-\eps) \left(\frac{1}{2} - 4 \eps -2 \kappa \right) \frac{1}{\tilde{\Lambda}} \ .
\end{align}
Using the bound~\eqref{ineq:hyperconcentration} for $\theta=\frac{1}{2}$, we obtain
\begin{align*}
    \pr{\sum_{t=1}^T \eta^-_t \geq \frac{1}{4\delta' \tilde{\Gamma}}} &\geq \frac{1}{4} \cdot \frac{T \cdot \ex{\eta_t^-}^2}{\Var(\eta_t^-) + T \cdot \ex{\eta_t^-}^2} \overset{(1)}{\geq} \frac{1}{4} \cdot \frac{T \cdot \ex{\eta_t^-}^2}{\frac{2}{1+\frac{\tilde{\Gamma}}{2}} \cdot \ex{\eta_t^-} + T \cdot \ex{\eta_t^-}^2}  \\ &\geq \frac{1}{4} \cdot \frac{1}{\frac{2}{T\ex{\eta_t^-} \cdot (1+{\tilde{\Gamma}}/{2})} + 1} \overset{(2)}{\geq} \frac{1}{4} \cdot \frac{1}{\frac{2\delta' \tilde{\Gamma}}{{(1/2 - 4\eps - 2\kappa)(1+\tilde{\Gamma}/2)}} + 1} \geq \frac{1}{4} \cdot \frac{1}{\frac{4}{(1/2-4\eps - 2\kappa)} \delta' + 1} \ ,
\end{align*}
where (1) uses \Cref{clm:nonbusy} and inequality \eqref{prop:core} and (2) uses inequality \eqref{ineq:z_bounds}. Concurrently, our tail bound~\eqref{ineq:expconcentration} for sum of exponential distributions gives
\begin{eqnarray} \label{ineq:T}
    \pr{\sum_{t=1}^T \eta^+_t\geq \frac{2}{\delta' \tilde{\Gamma}}} \leq \frac{1}{2}  e^{-T(1 -\ln 2)} \leq \frac{1}{2} e^{-\frac{(1/4 - 2\eps - \kappa)(1 -\ln 2)}{\delta'}} \ .
\end{eqnarray}
We choose $\delta'$ such that $\frac{1}{\delta'} =  \frac{t_i \tilde{\Gamma}}{4} \geq \frac{1}{4\delta}$. Therefore, with probability of at least 
\[ \frac{1}{4} \cdot \frac{1}{\frac{16}{(1/2-4\eps - 2\kappa)} \delta + 1} - e^{-\frac{(1 - 8\eps - 4\kappa)(1 -\ln 2)}{\delta}} 
\] we have $\sum_{t = 1}^T \eta_t^+ \leq \frac{2}{\delta' \tilde{\Gamma}} = \frac{t_i}{2}$ and $\sum_{t = 1}^T \eta_t^- \geq \frac{1}{4\delta'\tilde{\Gamma}} = \frac{t_i}{16}$. Assuming these conditions, we now argue that 
\begin{align*}
    \sum_{k\in J^{\rm correl}\cap N_i} \gamma_k\delta_{i,k} &\leq \max\left\{ t_i \tilde{\Gamma} - \left(t_i - \sum_{t=1}^T \eta_t^+\right) \cdot \frac{\tilde{\Gamma}}{2}, t_i \tilde{\Gamma} - \left(\sum_{t=1}^T \eta_t^-\right) \cdot \frac{\tilde{\Gamma}}{2}\right\} \\ & \leq \tilde{\Gamma} \cdot \max\left\{ \frac{3t_i}{4}, \frac{31t_i}{32}\right\} = \frac{31}{32} t_i \tilde{\Gamma}
     \ , 
\end{align*}
where the first argument in the max expression follows from assuming that $t_i$ was exceeded after the $T$ blocked and non-blocked cycles. In this case, at any moment $t$ at which $I^{\rm core}$ is not blocked, we have $\sum_{k \in J^{\rm correl} \cap N_i} \gamma_k \psi_k(t) \leq \frac{\tilde{\Gamma}}{2}$ by inequality \eqref{prop:core}. Observing that this non-blocked time length is at least  $t_i - \sum_{t=1}^T \eta_t^+ \geq \frac{t_i}{2}$ gives the first argument. The second argument corresponds to the reverse case that $t_i$ exceeds the $T$ pairs of cycles in which the non-blocked time length is at least $\sum_{t=1}^T \eta_t^- \geq \frac{t_i}{16}$. Having $\delta$ small enough proves the lemma with $c_0 = 1/32$ and $c_1 = {1}/{8}$. 

\paragraph{Case 2: $\boldsymbol{{\sum_{k\in J^{\rm correl}\cap N_i}\gamma_k} < \frac{4}{1-\ln 2}}$.} The proof in this case follows the same approach as in case 1, however, we use the notion of blocked periods for a different set of offline vertices. Fix an arbitrary $k\in J^{\rm correl}\cap N_i$. Consider $T = \lceil (\sum_{i' \in S_k^\uparrow}\lambda_{i'})/\delta')\rceil \geq \frac{1-\eps}{2\delta'}$ blocked and non-blocked cycles of $S_k^\uparrow$, which we denote by $\eta^+_1,\eta^-_1,\ldots,\eta^+_T,\eta^-_T$ \footnote{The lower bound for $T$ comes from the fact that $\sum_{i' \in S_k^\uparrow} \lambda_{i'} \geq \sum_{i' \in S_k^\uparrow} x_{i', a} \geq \frac{1-\eps}{2}$.}. The cycles from each type are  i.i.d. with $\eta^+_1 \sim Exp(\sum_{{i'} \in S_k^\uparrow}\lambda_{i'})$ and $\eta^-_1\succeq Z$ where $Z$ is defined as in Claim~\ref{clm:nonbusy} (with $I = S_k^\uparrow$). Using inequality~\eqref{ineq:hyperconcentration} with $\theta=\frac{1}{2}$ and Claim~\ref{clm:nonbusy}, we obtain
\begin{eqnarray} \label{ineq:neg2}
    \pr{\sum_{t=1}^T \eta^-_t\geq \frac{1}{4\delta'}} \geq (1-\theta)^2 \cdot \frac{1}{\frac{2}{T\expar{\eta^-_t}} + 1} \geq \frac{1}{4(2\delta'+1)} \ .
\end{eqnarray}
Concurrently, our tail bound~\eqref{ineq:expconcentration} for sum of exponential distributions gives
\begin{eqnarray} \label{ineq:T2}
    \pr{\sum_{t=1}^T \eta^+_t\geq \frac{2}{\delta'}} \leq e^{-\frac{1-\eps}{2\delta'}(1 -\ln 2)} \ ,
\end{eqnarray}
Choosing $\frac{1}{\delta'} = \frac{\tau_i}{4} \geq \frac{1}{\delta((1-\ln 2)}$ because of the case hypothesis and the assumption in Lemma~\ref{lem:correl} that $\tau_i\geq \frac{1}{\delta}\min\{\frac{1}{ (\sum_{k\in J^{\rm correl}\cap N_i}\gamma_k)},\frac{4}{(1-\ln 2)}\} = \frac{4}{\delta (1-\ln 2)}$. Then, with probability $\frac{1}{4(1+2(1-\ln 2)\delta)}-\eps^{\frac{1}{\delta}}$, we have
\begin{eqnarray} \label{bound:single}
    \gamma_k\delta_{i,k} &\leq& \max\left\{ \gamma_k\frac{\tau_i}{2},  \gamma_k \tau_i - \gamma_k  \left(\sum_{t=1}^T \eta_t^-\right) \right\} 
    \leq \gamma_k\max\left\{\frac{\tau_i}{2},\frac{15\tau_i}{16} \right\} = \gamma_k\frac{15\tau_i}{16} \ ,
\end{eqnarray}
where the first term in the max-expression follows from inequality~\eqref{ineq:T2} assuming that $\tau_i$ was exceeded after $T$ busy and non-busy cycles and the right term holds for the reverse case. The second inequality follows from~\eqref{ineq:neg2}.

To conclude, observe that
\begin{eqnarray*}
    \pr{\sum_{k\in J^{\rm correl}\cap N_i} \gamma_k\delta_{i,k}\geq \frac{127}{128} \sum_{k\in J^{\rm correl}\cap N_i} \gamma_k\tau_i} &\leq & \frac{\expar{\sum_{k\in J^{\rm correl}\cap N_i} \gamma_k\delta_{i,k}}}{\frac{127}{128} \sum_{k\in J^{\rm correl}\cap N_i} \gamma_k\tau_i} \\
    &\leq & \frac{(\frac{63}{64}+\eps+\delta)\sum_{k\in J^{\rm correl}\cap N_i} \gamma_k\tau_i}{\frac{127}{128} \sum_{k\in J^{\rm correl}\cap N_i} \gamma_k\tau_i} \\
    &=& \frac{126}{127} +\frac{128}{127} (\eps+\delta) \ ,
\end{eqnarray*}
where the first inequality is derived from Markov inequality, and the second inequality is a consequence of~\eqref{bound:single} for sufficiently small $\delta$. This gives the desired bound.
% \Alicomment{Easier case: we show concentration for each $\delta_{i,k}$ by a large time $M$.}
% By definition of $J^{\rm correl}$, we have
% \begin{eqnarray*}
% \sum_{i\in S_j^\uparrow \cap S_k^\uparrow} \frac{\lambda_i}{ \sum_{i\in S_j^\uparrow}\lambda_i} \cdot \frac{1}{1+\sum_{l\in N_k} \gamma_j}\geq \left(\frac{1}{2}-\eps-\kappa \delta\right) \frac{1}{\sum_{i\in S_j^\uparrow}\lambda_i}
% \end{eqnarray*}

% Suppose that $S_j^\uparrow = S_k^\uparrow$ for all $k\in J^{\rm correl}\cap N_i$. \Alicomment{At the moment, I am not sure how to bypass this assumption. We know that they overlap a lot, I assume exact overlap.}

% Consider $T = \lceil (\sum_{b \in S_j^\uparrow}\lambda_b)/({\sum_{k\in J^{\rm correl}\cap N_i}\gamma_k})\rceil$ busy and non-busy cycles, which we denote by $\eta^+_1,\eta^-_1,\ldots,\eta^+_T,\eta^-_T$. From the time-reversibility of the top vMc queues, we go backwards in time from $t^\infty$, starting initially from a busy cycle. The cycles from each type are i.i.d. with $\eta^+_1\sim Exp(1+\sum_{b \in S_j^\uparrow}\lambda_b)$ and $\eta^-_1 \succeq Z$ from Claim~\ref{clm:nonbusy}.

% Note that we can write
% \begin{eqnarray}\label{eq:decomposition}
% \ex{\sum_{k\in J^{\rm correl}\cap N_i}\gamma_k(\tau_i-\delta_{i,k}) | t_i = \tau_i,\psi_j(t^\infty) =1} = \sum_{c=1}^\infty \ex{ \min\left\{\eta^-_c,\max\left\{0,\tau_i - \sum_{f<c} (\eta^+_f +\eta^-_f) \right\}\right\}}
% \end{eqnarray}

% % \begin{fact} The RHS  is a non-decreasing concave function in the distribution of $\eta^-_1$. \end{fact}

% % \begin{proof}

% % \end{proof}


% The worst-case distribution for the duration of non-busy cycles is bimodal. Inequality \eqref{ineq:difficult_type2} implies that with constant probability after such many cycles, the non-busy cycle starts with $a\in S_j^\uparrow$ such that $1+\sum_{k \in N_a} \gamma_k \leq 2\sum_{k\in J^{\rm correl} \cap N_i} \gamma_k {\bb I}[a\in S_k^\uparrow] \leq 2\sum_{k\in J^{\rm correl} \cap N_i} \gamma_k$. The next non-busy cycle is exponentially distributed  conditional on the history with mean distribution $(2\sum_{k\in J^{\rm correl} \cap N_i} \gamma_k)^{-1}$ in expectation but the cumulative time so far at the beginning of the non-busy cycle is also at most $\eta T\cdot \frac{1}{\sum_{b \in S_j^\uparrow}\lambda_b} = \frac{\eta}{\sum_{k\in J^{\rm correl}\cap N_i}\gamma_k}$ with proba $e^{1-\eta}$ for every $\eta>1$.
\end{proof}

\begin{lemma} \label{lem:rand}
There exist constants $c_2,c_3 \in (0,1)$ such that for each $i \in S_j^\downarrow$, we have 
% $\prpar{\delta_{i,k} \geq (1-c_1) \tau_i  | t_i = \tau_i,\psi_j(t^\infty) =1} \leq 1-c_2$, implying 
% $\expar{\sum_{k\in J^{\rm indep}\cap N_i}\gamma_k\delta_{i,k} | t_i = \tau_i,\psi_j(t^\infty) =1} \leq (1-c_1) \sum_{k\in J^{\rm indep}\cap N_i}\gamma_k\tau_i $.
\[ 
\pr{\left.\sum_{k\in J^{\rm indep}\cap N_i}\gamma_k\delta_{i,k}\leq (1-c_2) \sum_{k\in J^{\rm indep}\cap N_i} \gamma_k t_i  \right| t_i,\psi_j(t^\infty) =1} \geq c_3 \ .
\]
\end{lemma}
\begin{proof}
    We prove the stronger result that for every $k \in J^{\rm indep} \cap N_i$, we have $\ex{\delta_{i,k}} \leq c'' \cdot \ex{t_i}$ for some constant $c'' > 0$. The lemma then follows from applying the Markov inequality.
    
    Consider some $k \in J^{\rm indep} \cap N_i$ and let $I^k = S_k^\uparrow \setminus S_j^\uparrow$ with $\sum_{i' \in I^k} x_{i', a} \geq \kappa_1 \delta$ from $k \in J^{\rm indep}$. Like before, we are interested in blocked times when $\sum_{i' \in I^k} Q_{i'}^s = 0$. Since $I^k \cap S_j^\uparrow = \emptyset$, the conditional probability given $\psi_j(t^\infty)$ coincides with the unconditional probability:
    \begin{align*}
        \pr{\sum_{i' \in I^k} Q_{i'}^s(t) = 0} = \exp\left(-\sum_{i' \in I^k} x_{i', a}\right) \leq \exp(-\kappa_1 \delta) \ , 
    \end{align*} for every time $t \geq 0$. Therefore, since queue $i$ is also independent of the state queues in $I^k$, we have 
    \begin{align*}
        \ex{\delta_{i,k}} = \int_{t^\infty - t_{i}}^{t^\infty} \pr{\sum_{i' \in I^k} Q_{i'}^s(t) = 0} dt \leq \exp(-\kappa_1 \delta) \cdot t_i \ .
    \end{align*}
    We thus obtain
    \begin{align*}
        \pr{\sum_{k \in J^{\rm indep} \cap N_i} \gamma_k \delta_{i,k} \geq \tilde{c} \cdot \exp(-\kappa_1 \delta) \cdot t_i \sum_{k \in J^{\rm indep} \cap N_i} \gamma_k } \leq \frac{\exp(-\kappa_1 \delta)}{\tilde{c}\exp(-\kappa_1 \delta)} = \frac{1}{\tilde{c}} \ .
    \end{align*}
    Letting $\tilde{c} = \frac{1}{\exp(-\kappa_1 \delta)} - \tilde{\eps}$ for some fixed $\tilde{\eps} \ll \frac{1}{\exp(-\kappa_1 \delta)}$ gives the desired result. 
    
    
    
    
%     \paragraph{Case 1: $\Gamma_i \geq \frac{4}{1-\ln2}$.} Consider some $k \in J^{\rm indep} \cap N_i$ and let $I^k = S_k^\uparrow \setminus S_j^\uparrow$ with $\sum_{i' \in I^k} x_{i', a} \geq \kappa_1 \delta$ from $k \in J^{\rm indep}$. Like before, we define blocked cycles as the ones where $\sum_{i' \in I^k} Q_{i'} = 0$ and non-blocked otherwise. Since $I^k \cap S_j^\uparrow = \emptyset$, the conditional probability given $\psi_j(t^\infty)$ coincides with the unconditional probability. Let $\delta'>0$ be an auxiliary parameter. Consider $T = \lceil (\sum_{i' \in I^k}\lambda_{i'})/(\delta')\rceil$ blocked and non-blocked cycles from time $t^\infty - t_i$, denoted by $\eta^+_1,\eta^-_1,\ldots,\eta^+_T,\eta^-_T$. We assume that at time $t^\infty - t_i$ we are at a blocked cycle; this assumption does not affect our result since it provides an upper bound for $\delta_{i,k}$ whereas it does not affect $t_i$. By \Cref{clm:nonbusy}, the cycles from each type are  i.i.d. with $\eta^+_1 \sim Exp(\sum_{i' \in I^k}\lambda_{i'})$ and $\eta^-_1\succeq Z$ where $Z$ is a hyperexponential distribution formed by the mixture $(p_{i'})_{i' \in I^k}$ with $p_{i'} = \frac{\lambda_{i'}}{\sum_{i'' \in I^k} \lambda_{i''}}$ of exponential distributions $Exp(1+\sum_{k \in N_{i''}} \gamma_k)$. \Cref{clm:nonbusy} gives $\ex{Z} \geq (1-\eps) \cdot \kappa_1 \delta \cdot \frac{1}{\sum_{i' \in I^k} \lambda_i} \geq 1-\eps$ and $\ex{Z^2} \leq $ and using inequality~\eqref{ineq:hyperconcentration} with $\theta=\frac{1}{2}$, we obtain
% \begin{align*}
%     \pr{\sum_{t=1}^T \eta^-_t \geq \frac{1}{2} \cdot \frac{(1-\eps)\kappa_1 \delta}{\delta'}} &\geq \frac{1}{4} \cdot \frac{T \cdot \ex{\eta_t^-}^2}{\Var(\eta_t^-) + T \cdot \ex{\eta_t^-}^2} \geq \frac{1}{4} \cdot \frac{T \cdot \ex{\eta_t^-}^2}{2\ex{\eta_t^-} + T \cdot \ex{\eta_t^-}^2} \geq  \frac{1}{4} \cdot \frac{\frac{(1-\eps)\kappa_1 \delta}{\delta'}}{2 + \frac{(1-\eps)\kappa_1 \delta}{\delta'}} \\ &= \frac{1}{4} \cdot \frac{1}{\frac{2\delta'}{(1-\eps)\kappa_1 \delta} + 1} 
% \end{align*}
% Concurrently, our tail bound~\eqref{ineq:expconcentration} for sum of exponential distributions gives
% \begin{eqnarray} \label{ineq:T2}
%     \pr{\sum_{t=1}^T \eta^+_t \geq  \frac{2}{\delta'}} \leq \frac{1}{2} e^{-T(1 -\ln 2)} = \frac{1}{2} e^{-\frac{\sum_{i' \in I^k} \lambda_{i'}}{\delta'} \cdot (1-\ln 2)} \leq \frac{1}{2} e^{-\frac{\kappa_1 \delta}{\delta'} \cdot (1-\ln 2)} \ .
% \end{eqnarray}
% Let $\delta'' = \frac{\delta'}{\Gamma_i}$. We now choose $\delta' = \frac{4}{t_i}$ and so $\delta''$. If $\Gamma_i \geq \frac{4}{1-\ln2}$, we have $\frac{1}{\delta'} = \frac{t_i}{4} \geq \frac{1}{4\Gamma_i \cdot \delta} \geq \frac{1-\ln 2}{\delta}$. Otherwise, we have $\frac{1}{\delta'} = \frac{t_i}{4} \geq $

% Our choice of $\delta'$ depends on the value of $\Gamma_i$. If $\Gamma_i \geq \frac{4}{1-\ln2}$, we choose $\delta'$ such that $\frac{1}{\delta'} =  \frac{t_i}{4} \geq \frac{1}{\delta}$ and $\frac{1}{\delta'} = \frac{t_i}{2} \geq \frac{2/(1-\ln 2)}{\delta}$ otherwise.

% Then, with probability xxx, we have $\sum_{t = 1}^T \eta_t^+ \leq \frac{2}{\delta'} = \frac{t_i}{2}$ and $\sum_{t = 1}^T \eta_t^- \geq \frac{(1-\eps)\kappa_1 \delta}{2} \cdot \frac{1}{\delta'} = \frac{(1-\eps)\kappa_1 \delta}{8} \cdot t_i$. We now argue that 
% \begin{align*}
%     \gamma_k\delta_{i,k} \leq \max\left\{ \gamma_k\frac{\tau_i}{2},  \gamma_k \tau_i - \gamma_k  \left(\sum_{t=1}^T \eta_t^-\right) \right\} 
%     \leq \gamma_k\max\left\{\frac{\tau_i}{2},\frac{15\tau_i}{16} \right\} = \gamma_k\frac{15\tau_i}{16} \ ,
% \end{align*}
% where the first argument in the max expression follows from inequality~\eqref{ineq:T2} assuming that $t_i$ was exceeded after $T$ blocked and non-blocked cycles. In this case, we clearly have 
% \[
%     \delta_{i,k} \leq \sum_{t=1}^T \eta_t^+ \leq \frac{t_i}{2} \ .
% \] 
% The latter argument in the max expression corresponds to the opposite case where $t_i$ exceeds the $T$ blocked and non-blocked cycles in which case we have 
% \[ 
%     \delta_{i,k} \leq t_{i} - \sum_{t=1}^T \eta_t^- \leq t_i - \frac{(1-\eps)\kappa_1 \delta}{8} \cdot t_i \ .
% \] 
% We now choose $\delta' = \frac{4 \delta \tau_i^*}{t_i} \leq 4\delta$. We want
\end{proof}

Lemma~\ref{lem:main} follows from combining Lemmas~\ref{lem:correl} and~\ref{lem:rand}. We distinguish between two cases. If $\sum_{k\in J^{\rm correl}\cap N_i} \gamma_k \geq \frac{1}{2}\sum_{k\in  N_i} \gamma_k$, then Lemma~\ref{lem:main} holds for $c = c_0/2$ and $\bar{c} = c_1$. Conversely, if $\sum_{k\in J^{\rm indep}\cap N_i} \gamma_k = \sum_{k\in  N_i} \gamma_k- \sum_{k\in J^{\rm correl}\cap N_i} \gamma_k >  \frac{1}{2}\sum_{k\in  N_i} \gamma_k$ then Lemma~\ref{lem:main} holds for $c = c_2/2$ and $\bar{c} = c_3$.
